ConMax: Confidence-Maximizing Compression for Efficient Chain-of-Thought Reasoning

Recent breakthroughs in Large Reasoning Models (LRMs) have demonstrated that extensive Chain-of-Thought (CoT) generation is critical for enabling intricate cognitive behaviors, such as self-verification and backtracking, to solve complex tasks. However, this capability often leads to ``overthinking'', where models generate redundant reasoning paths that inflate computational costs without improving accuracy. While Supervised Fine-Tuning (SFT) on reasoning traces is a standard paradigm for the 'cold start' phase, applying existing compression techniques to these traces often compromises logical coherence or incurs prohibitive sampling costs. In this paper, we introduce ConMax (Confidence-Maximizing Compression), a novel reinforcement learning framework designed to automatically compress reasoning traces while preserving essential reasoning patterns. ConMax formulates compression as a reward-driven optimization problem, training a policy to prune redundancy by maximizing a weighted combination of answer confidence for predictive fidelity and thinking confidence for reasoning validity through a frozen auxiliary LRM. Extensive experiments across five reasoning datasets demonstrate that ConMax achieves a superior efficiency-performance trade-off. Specifically, it reduces inference length by 43% over strong baselines at the cost of a mere 0.7% dip in accuracy, proving its effectiveness in generating high-quality, efficient training data for LRMs.

==> sections/0_introduction_old.tex <==
\section{Introduction}
% Background
Large Reasoning Models (LRMs) such as O1 and R1, have achieved remarkable performance on reasoning-intensive tasks such as mathematics competitions and code generation. This success is largely due to their ability to develop detailed chains of thought (CoT), which enable comprehensive analysis of problems before reaching a final answer. However, while these extended reasoning trajectories have been proven effective, their length—often spanning thousands or even tens of thousands of tokens—introduces non-negligible inference overhead. Underneath these lengthy  CoT, recent research has revealed that the thinking trajectories tend to be verbose, with models engaging in excessive reasoning even for simple questions. 


% 思维链的本质, 目前方法的局限 lack of citation 
% Recap, TBD later
% 2025 EMNLP: ConCISE
Compressing lengthy chains of thought and fine-tuning models using these compressed thought chains can enhance a model’s reasoning ability, thereby improving its performance on downstream reasoning tasks while maintaining a certain level of inference efficiency. A typical reasoning trajectory is similar to human thought processes, usually involving fundamental steps such as sub-problem solving, exploration, verification, error correction, and backtracking. These components are interwoven in unpredictable ways, resulting in lengthy thought chains that often contain redundant information. This complexity makes it challenging to identify and effectively compress unnecessary parts. Some existing studies attempt to segment the original thought chain using heuristic rules based on length, retaining only parts of the chain (such as the segment containing the first correct solution) as the compressed thought chain. However, such methods often disrupt the original structure of the thought chain, limiting the model’s ability to learn complex reasoning patterns and thus affecting overall performance. Another category of search-based compression methods iteratively optimizes each step in the thought chain to obtain a more concise reasoning path. While this approach may plausibly find better solutions, it requires searching at every step, which results in extremely high sampling costs; moreover, the compressed chains often remain relatively long, so the overall compression efficiency is still limited in practice.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/length_stds_ans_consistency.pdf}
    \caption{Comparison of Length Standard Deviation Distribution and Answer Consistency Ratio. Write specific description. }
    \label{fig:placeholder}
\end{figure}

% learning-based compression is not trival, our insight, why the method can work. Move method motivation here
Model-based compression of chains of thought, in theory, offers more flexibility than heuristic or search-based methods. It can adapt to the complex structure of reasoning trajectories, automatically identify redundancies, and preserve the essential logical steps—potentially leading to more effective compression and reduced inference overhead. However, model-based compression is far from trivial and faces two main challenges. First, while today’s large models have powerful reasoning and comprehension abilities, generating high-quality compressed reasoning chains on-the-fly via simple instruction prompts often demands skillful and case-specific prompt engineering. The entangled and intricate nature of reasoning chains makes prompt tuning particularly challenging, and the overall compression quality remains tightly coupled with the model’s own capabilities. Second, evaluating the quality of compressed chains of thought is inherently difficult. Unlike summarization tasks—where the compressed text is itself the final product—reasoning chains serve only as intermediate steps toward a final answer.
\paragraph{Method Motivation}
\md{[change this]} For a given problem $x$, a large reasoning model can generate multiple valid reasoning trajectories ${z_i}_{i=1}^k$, each of which leads to the same correct answer $y$. To quantitatively validate this observation, we empirically analyze around 9k math problems from the NuminaMath dataset. Using the R1-Distill-Qwen-7B\footnote{https://huggingface.co/deepseek-ai/DeepSeek-R1-Distill-Qwen-7B} (shorted as R1-7B below), we employ rejection sampling to generate $k=8$ candidate solutions for each problem $x$, ensuring that all sampled reasoning trajectories ${z_i}$ resulted in the correct answer $y$. We use the token length $|z_i|$ of each reasoning trajectory as a proxy for its information redundancy. For each problem, we compute the standard deviation of the token lengths ${|z_i|}_{i=1}^k$ across the sampled reasoning trajectories. As illustrated in the top panel of Figure 1, the distribution of these standard deviations reveals a large and widespread variance in the length of the reasoning trajectories. These observations imply that the model's reasoning processes may involve a notable degree of diversity and stochasticity, even if the final answer remains consistent. In contrast, the final answer length $|y|$ is much more consistent, with a far smaller standard deviation than that of the reasoning chain $|z|$.

Using inference-time strategies to discover more succinct reasoning paths comes with significant trade-offs. Approaches like repeated sampling and Monte Carlo search necessitate multiple forward passes, which incur substantial computational cost and latency. Their stochastic nature also means they cannot be relied upon to consistently find optimal solutions. To overcome these challenges, this paper explores how to internalize the search for optimal reasoning paths into the model’s parameters. Specifically, we aim to develop a self-guided training method that enables the model itself to generate concise and efficient reasoning chains in a single forward pass. This approach seeks to avoid the high computational demands of online search while improving both the stability and quality of generated reasoning paths without compromising accuracy.

% \begin{wrapfigure}{r}{0.4\textwidth}
%   \centering
%   \includegraphics[width=0.4\textwidth]{figures/length_stds_ans_consistency.pdf}
%   \caption{Comparison of Length Standard Deviation Distribution and Answer Consistency Ratio. Write specific description. }
%   \label{fig:len_std}
% \end{wrapfigure}


\paragraph{Overview of Our Method and Its Efficacy}
\clearpage
